Approximation Algorithms for Probabilistic Graphs

We study the k-median and k-center problems in probabilistic graphs. We analyze the hardness of these problems, and propose several algorithms with improved approximation ratios compared with the existing proposals.

==> 0-command.tex <==
\def\done{\hspace*{\fill} {$\square$}}
\def\header{\vspace{2.5mm} \noindent}
\def\extraspacing{\vspace{2mm}}
\def\myspacing{\vspace{2mm}}
\def\figcapup{\vspace{-2mm}}
\def\figcapdown{\vspace{-3mm}}
\def\tblcapup{\vspace{-0mm}}
\def\tblcapdown{\vspace{2mm}}
\def\tbldown{\vspace{-2mm}}
\def\tblup{\vspace{2mm}}
\def\codecapup{\vspace{-3mm}}
\def\codecapdown{\vspace{-2mm}}
\newcommand{\E}{{\mathbb E}\xspace}
%\newcommand{\ar}{{\widehat{\boldsymbol{\rho}}_s}\xspace}
%\newcommand{\qs}{{\mathbf{q}_s}\xspace}
%\newcommand{\rs}{{\boldsymbol{\rho}}_s\xspace}
%\newcommand{\rv}{{\boldsymbol{\rho}}_v\xspace}
%\newcommand{\rk}{\boldsymbol{\rho}^K_s\xspace}
\newcommand{\AG}{$\mathsf{AdaptGreedy}$\xspace}
\newcommand{\EP}{$\mathsf{EPIC}$\xspace}
\newcommand{\G}{\mathcal{G}}
\newcommand{\KM}{\mathit{KM}}
\newcommand{\KC}{\mathit{KC}}
\newcommand{\UB}{\mathit{UB}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\OPT}{\mathrm{OPT}}


\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}



\def\correspondingauthor{\footnote{Corresponding author.}}



